Randomized Block Adaptive Linear System Solvers

Randomized linear solvers randomly compress and solve a linear system with compelling theoretical convergence rates and computational complexities. However, such solvers suffer a substantial disconnect between their theoretical rates and actual efficiency in practice. Fortunately, these solvers are quite flexible and can be adapted to specific problems and computing environments to ensure high efficiency in practice, even at the cost of lower effectiveness (i.e., having a slower theoretical rate of convergence). While highly efficient adapted solvers can be readily designed by application experts, will such solvers still converge and at what rate? To answer this, we distill three general criteria for randomized adaptive solvers, which, as we show, will guarantee a worst-case exponential rate of convergence of the solver applied to consistent and inconsistent linear systems irrespective of whether such systems are over-determined, under-determined or rank-deficient. As a result, we enable application experts to design randomized adaptive solvers that achieve efficiency and can be verified for effectiveness using our theory. We demonstrate our theory on twenty-six solvers, nine of which are novel or novel block extensions of existing methods to the best of our knowledge.

==> section/convergence-base.tex <==
\subsection{Another Title} 

If we attempt to apply \cref{corollary-stopped-meany} iteratively, then we could produce a convergence result for randomized, block, adaptive solvers. However, we will face two challenges. 
\begin{remunerate}
\item The first challenge is that we need to ensure the finiteness of $\nu(j)$ at any $j+1 \in \mathbb{N}$. In doing so, we will ensure that the sequence $\lbrace \tau_j : j+1 \in \mathbb{N} \rbrace$, defined sequentially by $\tau_0 = 0$ and 
\begin{equation} \label{eqn-base-progress-points}
\tau_{j+1} = \tau_j + \nu(\tau_j) + 1,
\end{equation}
is well-defined. Then, we can apply \cref{corollary-stopped-meany} to show that $\innorm{y_{\tau_{j+1}}}_2 \leq \gamma_{j} \innorm{ y_{\tau_j}}_2$ where $\gamma_{j} \in [0,1)$.
\item The second challenge is to ensure that $\lbrace \gamma_j \rbrace$ does not converge to $1$ so that $y_{\tau_j} \to 0$, which will allow us to conclude that base RBASs converge to a solution by .
\end{remunerate}

\subsection{Algorithmic Assumptions, Probabilistic Statements} \label{subsection-probabilistic}
These two obstacles can be addressed using a multitude of assumptions about the algorithm encapsulated by $\varphi$ in \cref{eqn-row-adaptive,eqn-col-adaptive}, ranging from highly general to very specific. Our goal here is to strike a balance such that our theory covers a wide range of methods \textit{and} produces rates of convergence results that are minimally useful. Here, we view minimally useful rate of convergence results as being akin to their classical counterparts: namely, that after a fixed number of iterations (e.g., an entire run through the full set of equations), we are guaranteed a fractional reduction in the error. 

Accordingly, to address the first challenge, a direct translation of this latter requirement (based on \cref{corollary-stopped-meany} and the subsequent discussion) would entail making assumptions on the algorithm such that $\lbrace \nu(\tau_j) : j+1 \in \mathbb{N} \rbrace$ is uniformly bounded with probability one. However, such a requirement would unnecessarily limit the applicability of our results (e.g., we would have difficulty with Gaussian sketching methods). Instead, we will specify assumptions that imply $\sup_j \E{\nu(\tau_j)}$ is finite, which will address the first challenge.

In order to understand the provenance of these assumptions, we will need to collect a few facts about $\nu(j)$ (see \cref{eqn-nu-stop}). The first fact is to provide an upper bound for $\nu(j)$, which can be related to the geometry of the problem.


\cref{lemma-nu-upper-bound} allows us to bound $\nu(j)$ by studying the behavior of the non-decreasing sequence of spaces, $\lbrace \inlinspan{ y_j,\ldots,y_{j+k} } : k+1 \in \mathbb{N} \rbrace$, which has a natural upper bound (loosely, a space of dimension $\rnk A$). Therefore, so long as $\chi_{j+k} \neq 0$ enough times within a finite number of iterations, then $\nu(j)$ must be finite. Importantly, given that we use the stopping time, $\nu(\cdot)$, at multiple, random times to characterize the progress of the algorithm (see \cref{eqn-base-progress-points}), we will want $\nu(j)$ to be finite for any arbitrary $j$ and any possible value of the iteration, $y_j$. Importantly, the behavior of $\nu(j)$ can be highly dependent on the entire history of the iterates, $\lbrace y_i : i+1 \in \mathbb{N} \rbrace$, which would render establishing its finiteness particularly challenging. To ameliorate this issue, we will require the solvers to be forgetful, which, to our knowledge, is always the case in practice.  This notion of forgetful, formally called Markovian, is defined after we establish some notation. 


 Thus, with an abuse of notation, we can consider any Markovian RBAS to satisfy
\begin{equation}
\condPrb{ W_k \in \mathcal{W}, \zeta_k \in \mathcal{Z}}{\mathcal{F}_{k+1}^k} = \condPrb{ W_k \in \mathcal{W}, \zeta_k \in \mathcal{Z}}{\mathcal{F}_1^k}.
\end{equation}

Now that our procedure is forgetful, we need to ensure that it will produce a $\chi_j \neq 0$ at some point in the future. We achieve this with the notion of an exploratory RBAS, which we first state and then restated in terms of the common formulation, \cref{eqn-base-common-update}.


\begin{remark}
We may be tempted here to find a minimal $N$ or maximal $\pi$ for an $N,\pi$-Exploratory RBAS. However, we will see that this may not be optimal as the quantity that we be most important is $N/\pi$.
\end{remark}

\begin{lemma} \label{lemma-n-pi-exploratory-common}
A row-action RBAS (resp. column-action) is $N,\pi$-Exploratory if and only if for some $N \in \mathbb{N}$ and $\pi \in (0,1]$ if for all $V \subsetneq \row(A)$ (resp. $V \subsetneq \col(A)$)
\begin{equation}
\sup_{\substack{ y_0 \in V \\ \zeta_{-1}}} \condPrb{ \bigcap_{j=0}^{N-1} \left\lbrace \col(Q_j) \perp V \right\rbrace }{\mathcal{F}_1^0} \leq 1- \pi.
\end{equation}
\end{lemma}

Taken together, for an $N,\pi$-Exploratory, Markovian RBAS, we can guarantee that $\nu(j)$ is finite for an arbitrary choice of $j$.


\begin{corollary}
Under the setting of \cref{theorem-nu-finite}, the sequence $\lbrace \tau_{j}: j+1 \in \mathbb{N} \rbrace$ defined in \cref{eqn-base-progress-points} satisfies one of the following alternatives:
\begin{remunerate}
\item there exists a $j +1 \in \mathbb{N}$ such that $A x_{\tau_j} = b$ and for all $k \in [0,j] \cap \mathbb{N}$, $\E{ \tau_k } \leq k [ (\rnk{A} - 1) N/\pi + 1 ]$; or
\item for all $j +1 \in \mathbb{N}$, $\E{ \tau_j} \leq j [ (\rnk{A} - 1) N/\pi + 1 ]$.
\end{remunerate}
\end{corollary}
\begin{proof}
The proof proceeds by induction. For $j=0$, recall $\tau_0 = 0$. Now, either $Ax_{\tau_0} = b$ or $Ax_{\tau_0} \neq b$. In the former case, the statement of the result is true. In the latter case, $\tau_1 = \nu(\tau_0) + 1$ is finite with probability one and $\E{ \tau_1} \leq (\rnk{A} - 1) N/\pi + 1$ by \cref{theorem-nu-finite}. Therefore, we see that the result holds for $j=0$. For the induction hypothesis, suppose that for $j \in \mathbb{N}$, $A x_{\tau_{j-1}} \neq b$ and $\E{ \tau_{k}} \leq k [ (\rnk{A} - 1) N/\pi + 1]$ for $k \in [0,j-1]\cap\mathbb{N}$. To conclude, by \cref{theorem-nu-finite}, $\tau_j = \tau_{j-1} + \nu(\tau_{j-1}) + 1$ is finite and $\E{\tau_{j}} \leq (j-1) [ (\rnk{A} - 1) N/\pi + 1] + (\rnk{A} - 1) N/\pi + 1 = j[ (\rnk{A} - 1) N/\pi + 1]$. Finally, either $Ax_{\tau_{j}} = b$ or $Ax_{\tau_{j}} \neq b$. The result follows.
\end{proof}

We now move onto the second challenge. The first situation provides an important 

==> section/convergence-intro.tex <==
We now explore the convergence properties of the preceding methods summarized in \vp{table reference}. In \cref{subsection-convergence-base}, we will show that base RBASs that satisfy several simple properties will produce methods that converge and that will do so in finite time or at an exponential rate. In \cref{subsection-convergence-full}, we will show that RBASs with orthogonalization will converge in finite time. In \cref{subsection-convergence-oblique}, we will show that oblique RBASs will converge to a solution, but we will not provide a rate. Finally, in \cref{subsection-convergence-incomplete}, we will prove that base RBASs with incomplete solutions will converge, and supply a general convergence theory.
